Graph-Based Pulse Representation for Diverse Quantum Control Hardware

Pulse-level control of quantum systems is critical for enabling gate implementations, calibration procedures, and Hamiltonian evolution which fundamentally are not supported by the traditional circuit model. This level of control necessitates both efficient generation and representation. In this work, we propose pulselib - a graph-based pulse-level representation. A graph structure, with nodes consisting of parametrized fundamental waveforms, stores all the high-level pulse information while staying flexible for translation into hardware-specific inputs. We motivate pulselib by comparing its feature set and information flow through the pulse layer of the software stack with currently available pulse representations. We describe the architecture of this proposed representation that mimics the abstract syntax tree (AST) model from classical compilation pipelines. Finally, we outline applications like trapped-ion-specific gate and shelving pulse schemes whose constraints and implementation can be written and represented due to pulselib's graph-based architecture.

==> content/30_background.tex <==
\section{Background}
\label{sec:background}

\subsection{High-Level Pulse Representations}
\label{subsec:pulse_hll}
Currently, the most popular high-level representation used for pulses is Qiskit Pulse. Qiskit pulse is an abstract pulse representation primarily targeting superconducting quantum technologies and uses a sample-based model, which immediately suggests \acp{awg} are the target control equipment.
Measurement of the quantum state is also described at the pulse level, and classical operations such as arithmetic and control flow are not supported. However, in ~\cite{alexander2020qiskit}, the authors do mention that Qiskit pulse can be embedded in a larger instruction set to support classical arithmetic and control flow. This allows Qiskit pulse to be integrated into a larger software stack with an \ac{ir}, like \texttt{pulseIR}, to translate into appropriate pulse hardware interfaces. More recently, Qiskit Symbolic Pulse~\cite{Qiskit} was introduced as a parameterized pulse representation using symbolic expressions and parameters. Unlike Qiskit pulse, this is not sample-based, allowing it to function as a truly abstract high-level representation of parameterized pulses using envelop functions to describe the waveform.
However, it can only be translated into sample-based representations, and the lack a native set of fundamental blocks makes translation to other hardware control platforms challenging.

Other widely used pulse representations include Q-CTRL~\cite{boulder_opal1}, Pulser~\cite{pulser}, and JaqalPaw~\cite{lobser2023jaqalpaw}. Q-CTRL is a package used to generate optimized control pulses for trapped-ion quantum systems. Pulser is focused on neutral-atom arrays and uses a sample-based model, similar to Qiskit. Measurements in Pulser are discrete operations, but no classical operations are supported. Pulser includes features for pulse parameterization and working with composite (i.e. concatenated) pulses.
JaqalPaw uses a pulse-data model that exclusively targets their Octet coherent control hardware~\cite{clark2021engineering, lobster2022performant} which is developed for trapped ion quantum systems. Pulses defined with JaqalPaw can be used in Jaqal~\cite{landahl2020jaqal}, which is an assembly-like language for quantum kernels. Jaqal supports discrete operations for initialization and measurement but is not classically universal. JaqalPaw does include features that allow calibration parameters to be exposed through variables that can be used in pulse descriptions. 
% Calibration parameters have to be provided to compile and realize the described pulse. 

All of the above pulse representations are either too abstract, or too closely tied with  hardware representation. None of these are currently flexible enough to support all common control hardware systems which severely limits the flexibility of pulse programming or optimal control outputs - both the quantum hardware and the control hardware specifics require hand-optimized or technology-independent development. There is no unified pulse framework. We propose \texttt{pulseIR} to be this unifying piece in the software stack. High-level representations like Qiskit Pulse and Pulser can be compiled down to \texttt{pulseIR}, which can be further compiled down to hardware specific representations like JaqalPaw.

\subsection{Pulse Generation Hardware Interfaces}
\label{subsec:pulse_hw}
Generation of pulses for controlling quantum systems is done using signal generators. These are analog or digital devices that are used to generate electronic signals. Analog signal generators typically use a voltage-controlled oscillator (VCO) along with a phase locked loop (PLL) to generate analog signals. More recently, however, digital signal generators have become more popular owing to their accuracy and cost effectiveness. For the purpose of pulse control of quantum systems, types of digital signal generators can be divided into \acp{afg} and \acp{awg}. \acp{afg} have limited memory and use \ac{dds} to generate a limited set of waveforms like sine, square, pulse, ramp and sweep. 
%The use of \ac{dds} allows for precise generation of frequencies and quick switching between waveform frequencies. As \acp{afg} typically use \ac{dds} for signal generation, their input is a tuning word, which along with a reference clock generates the appropriate frequency. \acp{awg} on the other hand are able to generate any arbitrary waveform. The input to an \ac{awg} is typically a sample of points that make up the waveform and the resulting continuous waveform is generated using either a \ac{dds} or a variable clock generator. 
A very recent addition to this pulse generation landscape is the \ac{rfsoc} - an embedded system-on-chip platform for \ac{rf} signal generation. An \ac{rfsoc} can be configured to be more multi-tone \ac{dds}-like or more \ac{awg}-like. In either case, interfacing with an \ac{rfsoc} requires specialized software and gateware
% , like JaqalPaw for their Octet control hardware platform implemented on an \ac{rfsoc}.

The current popular hardware platforms have very different input interfaces, and none of the current high-level representations target \textit{all} these platforms. The lack of all-to-all support between these layers will only get worse with the development of newer representations and hardware platforms, which is expected as quantum computing is still in its relative infancy. \textbf{\texttt{pulseIR} aims to be an unifying \ac{ir} between these layers.}


==> content/80_integration.tex <==
\section{Integration: \texttt{pulseIR} as an IR}
\label{sec:pulse:integration}

\texttt{pulseIR} is a library focused on the representation of pulses, and practical usage requires integration into real-time quantum control systems and simulators. In this section, we discuss the integration of \texttt{pulseIR} into other systems.

For \texttt{pulseIR} to be used as an \ac{ir} it needs to be integrated as the target of \acp{hll} and as the source of low-level control systems and hardware systems. The former involves parsing the \ac{hll} and converting it into appropriate \texttt{pulseIR} nodes. If the high-level representation involves pulses across channels, these can be converted to a \texttt{pulseIR} schedule. 

Once the high-level representation has been translated to \texttt{pulseIR}, it can then be further integrated into a backend. These backends may be simulators or hardware accessed through control systems.
Quantum simulators that accept pulse-level input (e.g. Hamiltonian-level simulators based on QuTiP~\cite{JOHANSSON20121760, JOHANSSON20131234}, QuantumOptics.jl~\cite{kramer2018quantumoptics}, and IonSim.jl~\cite{ionsim}) can take \texttt{pulseIR} schedule objects as their input. The simulator provides channels and variables that can be used to create a schedule. The user-created schedule can be passed back to the simulator, which will pass it through a simulator-specific pipeline to obtain pulse descriptions in the desired format. Finally, the simulator can pass the pulse descriptions to the simulation backend to generate results for the user.
A schematic overview of the \texttt{pulseIR} integration into a simulator is shown in Figure~\ref{fig:pulse:sim}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/DAX - pulselib-sim-crop.pdf}
    \caption{Integration of \texttt{pulseIR} into a simulator.}
    \label{fig:pulse:sim}
\end{figure}

Similarly, quantum systems can provide pulse-level access to their hardware through real-time control systems using a \texttt{pulseIR} schedule as input. This input is initially hardware agnostic but can be passed to a device driver, which will transform the schedule to a device-specific
format. In this pipeline, the \texttt{pulsleib} schedule is first transformed to remove redundant nodes and simplify operations. It is then passed through a munch visitor which performs pattern matching over the graph and reduces it from a graph to a data structure compatible with the hardware interface. Finally, it is converted to the input accepted by the real-time pulse generator hardware and executed. For example, a \ac{dds} driver can convert the \texttt{pulseIR} \ac{ir} to \ac{dds} parameters that can be sent to the device in real-time. The device driver can perform any additional device initialization if required, such as uploading waveform data to external pulse generation equipment. The driver returns a handle that the user can store as part of a larger quantum program. Once the real-time part of the program is running, the user passes the handle to the device driver to play the desired pulse schedule. In this program, the execution of pulse schedules can be combined with classical operations and discrete quantum operations (e.g. state preparation and measurement) for classical and quantum complete kernels.
A schematic overview of the \texttt{pulseIR} integration into a real-time quantum control system is shown in Figure~\ref{fig:pulse:device}.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{fig/DAX - pulselib-device-crop.pdf}
    \caption{Integration of \texttt{pulseIR} into a real-time quantum control system. Only the ``Play'' process will be part of the real-time pulse generation on the hardware.}
    \label{fig:pulse:device}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/qiskit_pulse_ir.pdf}
    \caption{Pipeline demonstrating \texttt{pulseIR} as an \ac{ir} with a $\pi$-pulse written in Qiskit pulse as input. This pulse is a sine wave with a Gaussian envelope. High-level Qiskit representation is converted into a \texttt{pulseIR} graph comprised of a product node with a sine waveform multiplied by a discretized Gaussian waveform. This can be further automatically compiled down to 3 different hardware representations by \texttt{pulseIR} - an \ac{awg}, a \ac{dds} based \ac{afg}, and an \ac{rfsoc}.}
    \label{fig:ir:qiskit}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/qctrl_pulse_ir.pdf}
    \caption{Pipeline demonstrating \texttt{pulseIR} as an \ac{ir} with an amplitude-modulate piecewise-constant pulse written using Q-CTRL as input. The Q-CTRL representation is converted into a \texttt{pulseIR} graph comprised of a product node with a sine waveform multiplied by a sequence of constant waveforms. Like the Qiskit example, this is further compiled down automatically to 3 different hardware representations - an \ac{awg}, a \ac{dds} based \ac{afg}, and an \ac{rfsoc}.}
    \label{fig:ir:qctrl}
\end{figure*}

We demonstrate this pipeline of utilizing \texttt{pulseIR} as an \ac{ir} in Figures~\ref{fig:ir:qiskit} and \ref{fig:ir:qctrl}. In Figure~\ref{fig:ir:qiskit}, we take a Qiskit pulse as an input. This pulse represents a $\pi$-pulse, which executes an X gate. It is a sine wave whose amplitude is defined by a Gaussian envelope. This pulse is converted to a \texttt{pulseIR} representation which is a product node comprising of a sine node with the appropriate frequency, phase, and duration, multiplied with a Gaussian. This continuous Gaussian is discretized and represented as a sequence of constant waveforms. This is followed by \textit{an automated} translation to a hardware-specific representation. The ability to translate this graph representation to a variety of different hardware-specific inputs showcases the novelty and utility of \texttt{pulseIR} as an \ac{ir}. As seen in the demonstration, we have built pipelines to compile \texttt{pulseIR} down to \acp{awg}, \acp{afg} using \ac{dds}, and \acp{rfsoc}. The \ac{awg} takes a sample-based representation and is the one that is natively supported by Qiskit. An \ac{afg} that uses \ac{dds} takes its inputs as a frequency tuning word (ftw), an amplitude scale factor (asf), and a phase offset word (pow). These represent the frequency, amplitude, and phase respectively. Finally, the \ac{rfsoc} we used takes \texttt{PulseData}, a representation developed as part of JaqalPaw, as its input. Note, in this demonstration the \ac{rfsoc} output uses lower frequency and duration relative to the other platforms due to hardware restrictions on our particular \ac{rfsoc}. The demonstration shows the conversion of the Qiskit pulse to each of these formats. Figure~\ref{fig:ir:qctrl} shows a similar demonstration with an optimized amplitude-modulated piecewise-constant pulse from Q-CTRL as input. Here, too, the \texttt{pulseIR} \ac{ir} is a product node of a sine waveform and a sequence of constant waveforms. These demonstrations show the ability of \texttt{pulseIR} to be used as a target representation for different high-level pulse representations, while also being a source for a variety of pulse generation hardware platforms. As more such hardware platforms are used in quantum computing, the current \texttt{pulseIR} pipelines can be expanded to support these devices, while not burdening high-level representations.


==> minted_python3.tex <==
\setminted[python3]{fontsize=\footnotesize,frame=lines,framerule=\heavyrulewidth}

